On Lifting Integrality Gaps to SSEH Hardness for Globally Constrained CSPs

A $\mu$-constrained Boolean Max-CSP$(\psi)$ instance is a Boolean Max-CSP instance on predicate $\psi:\{0,1\}^r \to \{0,1\}$ where the objective is to find a labeling of relative weight exactly $\mu$ that maximizes the fraction of satisfied constraints. In this work, we study the approximability of constrained Boolean Max-CSPs via SDP hierarchies by relating the integrality gap of Max-CSP $(\psi)$ to its $\mu$-dependent approximation curve. Formally, assuming the Small-Set Expansion Hypothesis, we show that it is NP-hard to approximate $\mu$-constrained instances of Max-CSP($\psi$) up to factor ${\sf Gap}_{\ell,\mu}(\psi)/\log(1/\mu)^2$ (ignoring factors depending on $r$) for any $\ell \geq \ell(\mu,r)$. Here, ${\sf Gap}_{\ell,\mu}(\psi)$ is the optimal integrality gap of $\ell$-round Lasserre relaxation for $\mu$-constrained Max-CSP($\psi$) instances. Our results are derived by combining the framework of Raghavendra [STOC 2008] along with more recent advances in rounding Lasserre relaxations and reductions from the Small-Set Expansion (SSE) problem. A crucial component of our reduction is a novel way of composing generic bias-dependent dictatorship tests with SSE, which could be of independent interest.

==> corr-proof.tex <==
\section{Proof of Corollary \ref{corr:lift}}

Here we use Theorem \ref{thm:main} to prove Corollary \ref{corr:lift}. We begin by describing the $R$-round Sum-of-Squares relaxation of ${\sf SDP}_{\mu}(\psi)$ in the following figure:

\begin{figure}[ht!]
	\begin{mdframed}
		\begin{eqnarray*}
			\textnormal{Maximize} & \Ex_{e \sim w} \Pr_{X_e \sim \theta_e}\left[\psi(X_e) = 1\right] & \\
			\textnormal{Subject to} & \Ex_{i \sim V}\Pr_{X_i \sim \theta_i}\left[X_i = 1\right] = \mu &\\
			& \langle u_{A,\alpha},u_{B,\beta} \rangle = \Pr_{\theta_{A \cup B}}\left[X_A = \alpha, X_B = \beta\right] & 
			\forall~A,B \subseteq [R] \textnormal{such that} \\
			& & |A|,|B| \leq R/2, \\
			& & \alpha \in \{0,1\}^A, \beta \in \{0,1\}^B
	 \end{eqnarray*}
	\end{mdframed}
	\caption{${\sf SDP}_{\mu,R}(\psi)$}
	\label{fig:sos}
\end{figure}

The above SDP consists of local distributions $\{\theta_S\}_{|S| \leq R}$ for every $S \subseteq [R]$ of size at most $R$ -- these local distributions are consistent up to locality $R$ i.e., for any subset $A$ of size at most $R$, and any subset $B \subseteq A$, the $\theta_A$ when marginalized to the variables in $B$ must be identical to $\theta_B$. The inner product constraints ensure that the (pseudo)-moment matrix corresponding to the local distributions are positive semidefinite. We refer to any feasible solution to ${\sf SDP}_{R,\mu}(\psi)$ is a feasible $R$-round pseudo-distribution.

We begin with the following folklore smoothing lemma.

\begin{lemma}			\label{lem:smooth-1}
	The following holds for any $\eta \leq 1/r^2$. Given a  feasible $R$-round pseudo-distribution $\theta$, we can construct another feasible  $R$-round pseudo-distribution $\theta'$ such that 
	\[
	\Ex_{e \sim E_{\rm gap}}\Pr_{X_e \sim \theta'_e}\Big[\psi(X_e) = 1\Big] 
	\geq \Ex_{e \sim E_{\rm gap}}\Pr_{X_e \sim \theta_e}\Big[\psi(X_e) = 1\Big] - r\eta, 
	\] 
	and for every subset $S$ of size at most $r$ and $\alpha \in \{0,1\}^S$ we ahve 
	\[
	\Pr_{X_S \sim \theta_S}\Big[X_S = \alpha \Big] \geq \eta^r\mu^r.
	\]
\end{lemma}

\begin{proof}
	Given $\theta = \{\theta\}_{|S| \leq R}$, define $\{\theta'_S\}_{|S| \leq R}$ as follows. For every subset $S$ of size at most $R$, $\theta'_S$ corresponds to the following distribution: 
	\begin{itemize}
		\item Sample $X_S = (X_i)_{i \sim S}$ from the distribution $\theta_S$.
		\item For every $i \in S$, do the following independently: with probability $1 - \eta$, set $X'_i = X_i$, and with probability $\eta$ sample $X'_i \sim \{0,1\}_\mu$.
	\end{itemize}
	It is easy to verify that the resulting distribution is feasible and satisfies the inequalities claimed in the lemma.
\end{proof}

Furthermore, we shall need the following theorem from \cite{RT13} which shows that conditioning reduces average variance.

\begin{theorem}[Restatement of Theorem 4.1~\cite{RT13}]
	Let $\theta'$ be a $R$-round pseudo-distribution. Then for every $\eta' \in (0,1)$ small enough, there exists a subset $S$ of size at most $C/(\eta')^2$ and an assignment $\alpha \in \{0,1\}^S$, such that $\tilde{\theta} = \theta'| X_S \gets \alpha$ is a $R - |S|$ round feasible pseudo-distribution which satisfies
	\[
	\Ex_{i,j \sim V_{\rm gap}}\left[|{\rm Cov}_{\tilde{\theta}}(X_i,X_j)|\right] \leq \eta'.
	\]
\end{theorem}

Now we have all the ingredients required to prove Corollary \ref{corr:lift}.

\subsection{Proof of Corollary \ref{corr:lift}}

Let $G_{\rm gap} = (V_{\rm gap},E_{\rm gap},w)$ be an instance which satisfies the following:
\begin{itemize}
	\item The optimal value of ${\sf SDP}_{R,\mu}(\psi)$ on $G_{\rm gap}$ is $c$.
	\item ${\sf Opt}_\mu(G_{\rm gap}) = s$
\end{itemize}

Let $\theta$ be the $R$-round pseudo-distribution that achieves the optimal value of ${\sf SDP}_{R,\mu}(\psi)$. Let $\theta'$ be defined from $\theta$ as in Lemma \ref{lem:smooth-1}. Using Theorem \ref{thm:avg-corr}, we then construct $\tilde{\theta}|X_S \gets \alpha$. 


